Tunka Advanced Instrument for cosmic rays and Gamma Astronomy

The paper is a script of a lecture given at the ISAPP-Baikal summer school in 2018. The lecture gives an overview of the Tunka Advanced Instrument for cosmic rays and Gamma Astronomy (TAIGA) facility including historical introduction, description of existing and future setups, and outreach and open data activities.

==> Makefile <==
FILE = bss-taiga-2019 

PDFLATEX = pdflatex
BIBTEX = bibtex

PDF = ${FILE}.pdf

all :	
	${PDFLATEX} ${FILE}.tex
	${BIBTEX} ${FILE}
	${PDFLATEX} ${FILE}.tex
	${PDFLATEX} ${FILE}.tex

# Various cleaning options
clean :
	/bin/rm -f  *.log *.aux *.dvi *.bbl *.blg *.bm *.toc *.out \
	*Notes.bib *.ps

